Process-Aware Analysis of Treatment Paths in Heart Failure Patients: A Case Study

Process mining in healthcare presents a range of challenges when working with different types of data within the healthcare domain. There is high diversity considering the variety of data collected from healthcare processes: operational processes given by claims data, a collection of events during surgery, data related to pre-operative and post-operative care, and high-level data collections based on regular ambulant visits with no apparent events. In this case study, a data set from the last category is analyzed. We apply process-mining techniques on sparse patient heart failure data and investigate whether an information gain towards several research questions is achievable. Here, available data are transformed into an event log format, and process discovery and conformance checking are applied. Additionally, patients are split into different cohorts based on comorbidities, such as diabetes and chronic kidney disease, and multiple statistics are compared between the cohorts. Conclusively, we apply decision mining to determine whether a patient will have a cardiovascular outcome and whether a patient will die.

==> sections/0_limitations.tex <==
\section{\uppercase{Limitations}}
\label{sec:limitations}
\todo[inline]{MP: I'd propose to merge this section with the Conclusions section.}
In this study, we analyzed the treatment paths of patients.
However, the results have to be treated with caution. In the following, we investigate the reasons.

First, we do have a limited number of patients.
We only have records of 232 patients.
At the same time, we only have 942 events, i.e., roughly 4 events per patient in roughly two years.

Second, patients' data are sparse.
Sparse includes the temporal spareness that was former discussed, but also that not every attribute data has information for every patient.

Third, patients' data and their treatment are highly complex.
The data we analyzed only covers data recorded at the hospital.
It is not known if the treatments are in-between events at another hospital or which disease a patient had.
Depending on these, the overall state of a patient changes, yet it is not covered in the data.  
